Parsing Millions of DNS Records per Second

The Domain Name System (DNS) plays a critical role in the functioning of the Internet. It provides a hierarchical name space for locating resources. Data is typically stored in plain text files, possibly spanning gigabytes. Frequent parsing of these files to refresh the data is computationally expensive: processing a zone file can take minutes. We propose a novel approach called simdzone to enhance DNS parsing throughput. We use data parallelism, specifically the Single Instruction Multiple Data (SIMD) instructions available on commodity processors. We show that we can multiply the parsing speed compared to state-of-the-art parsers found in Knot DNS and the NLnet Labs Name Server Daemon (NSD). The resulting software library replaced the parser in NSD.

==> zoneother.tex <==


% Jeroen: grammar for various entries, probably not be entirely correct yet. Don't know if we
%         can use it, so commented out for now.
%<blank> ::= *WSP
%
%<item> ::= 1*contiguous / quoted
%
%<comment> ::= ";" *(WSP / VCHAR) CRLF
%
%<origin-control> ::= "\$ORIGIN" WSP item [WSP domain-name]
%
%<include-control> ::= "\$INCLUDE" WSP domain-name
%
%<ttl-control> ::= "\$TTL" WSP 1*DIGIT
%
%<custom-control> ::= "\$" 1*contiguous *(WSP item)
%
%<control> ::= origin-control / include-control / ttl-control / custom-control
%
%<labels> ::= 1*contiguous *("." 1*contiguous)
%
%<domain-name> ::= "@" / labels ["."]
%
%<ttl> ::= 1*DIGIT
%
%<mnemonic> ::= ALPHA *(ALPHA / DIGIT / "-")
%
%<class> ::= mnemonic / "CLASS" 1*5DIGIT
%
%<type> ::= mnemonic / "TYPE" 1*5DIGIT
%
%<rdata> ::= item *(WSP item)
%
%<rr> ::= [(ttl [1*WSP class] / class [1*WSP ttl]) 1*WSP] type WSP rdata
%
%<record> ::= domain-name WSP rr / 1*WSP rr
%
%<entry> ::= (blank / control / record) *comment CRLF


RFC1035~\cite{rfc1035} (section 5) defines the following entries:

\begin{verbatim}
<blank>[<comment>]
$ORIGIN <domain-name> [<comment>]
$INCLUDE <file-name> [<domain-name>] [<comment>]
<domain-name><rr> [<comment>]
<blank><rr> [<comment>]
\end{verbatim}

RFC2308~\cite{rfc2308} (section 4) additionally defines the following entry:

\begin{verbatim}
$TTL <TTL> [<comment>]
\end{verbatim}

Implementations typically interpret lines starting with a \$ (dollar-sign) as
a directive. Some implementations support custom directives. such as BIND supporting \$GENERATE.


Parenthesis cannot be nested!

now we go on to define the contents of <rr> like RFC1035.

\begin{verbatim}
[<TTL>] [<class>] <type> <RDATA>
[<class>] [<TTL>] <type> <RDATA>
\end{verbatim}

Here we note that the format is not context free. e.g. "IN" is fine for rdata
section in TXT RR, it is not for specifying the class

now we go on to state that the rdata section depends on the RR TYPE. And that
the content "The resource data or RDATA section of the RR are given using knowledge
of the typical representation for the data."

so the data is typed. i.e. "TTLs are integers" (RFC1034) TYPE and CLASS are
mnemonics (so not strings).

The labels in the domain name are expressed as character strings and
separated by dots.
>> so actually "foo"."bar".   >> not "foo.bar."
>> simdzone disallows quoted labels because name servers implement it differently
>> and nobody uses it. << an fine example of required knowledge of the dns.

note that for some fields, the items can be specified in multiple "items". e.g.
the base64 sequence in RRSIG RRs, it's not ok for defining strings in TXT RRs,
because "foo" "bar" is 3foo 3bar in wireformat, not 6foobar. There are
implementations that allow strings longer than 255 characters and cut them up
implicitly, but imho that's introducing more ambiguity.


now reference RFC3597~\cite{rfc3597} to include unknown type notation.

now reference RFC9460~\cite{rfc9460} to include the svcbparam notation. we must define
that it ever so slightly conflicts with the syntax rules established above
because based on that, the DQUOT starts a new item. Given that no white space
is allowed between the equals sign, we can hack around it.


%Master files and the corresponding textual representation of resources records were first introduced in RFC1034~\cite{rfc1034} (section 3.6.1) and RFC1035~\cite{rfc1035} (section 5), but the DNS has seen many additions since. The format is supported by commonly used names servers such as NSD, Knot, BIND and PowerDNS and provides operators with a standardized method of providing zone contents for the authoritative name server.

%Historically, master files were editted by hand, which is reflected in the syntax. The format is somewhat lax and allows for shorthand notation to avoid duplication. Apart from that, it must also cope with the intentional extensibility of the DNS. As a result, the format does not enforce any specific notation of data-types through syntax and the value of any field depends on it's relative location.

%Signature (security) relies on  base64.

%\url{https://fosdem.org/2023/schedule/event/dns_parsing_zone_files_really_fast/}


Describe here zone files.

But, why is it slow? Lex prefers longest prefix
Match multiple expressions (optimized?) Copy and unescape each token
Splits and rejoins labels (re)allocate, cat, repeat
Joins encoded data first

But, why is it still slow? Drop Lex and Yacc
Fields and order are (sort-of) fixed Cut (re)allocations
Maximum size 65535 bytes
Yields around ~180 MB/s (with mmap)
~700MB/s
Not context-free

\begin{verbatim}
$ORIGIN example.com.
$TTL 3660
example.com. IN 3600 SOA ns.example.com. hostmaster.example.com. (
                         2023020401 7200 3600 1209600 3600 )
; reuse owner (start with blank), class and ttl
A 192.0.2.1
; append origin (no trailing .) and reuse class
www 3600 A 192.0.2.1
; syntax error (start with blank), but no class or ttl
 mail A 192.0.2.1
; syntax error (did not start with blank), type is owner
A 192.0.2.1
\end{verbatim}


